ROOTS: Object-Centric Representation and Rendering of 3D Scenes

A crucial ability of human intelligence is to build up models of individual 3D objects from partial scene observations. Recent works achieve object-centric generation but without the ability to infer the representation, or achieve 3D scene representation learning but without object-centric compositionality. Therefore, learning to represent and render 3D scenes with object-centric compositionality remains elusive. In this paper, we propose a probabilistic generative model for learning to build modular and compositional 3D object models from partial observations of a multi-object scene. The proposed model can (i) infer the 3D object representations by learning to search and group object areas and also (ii) render from an arbitrary viewpoint not only individual objects but also the full scene by compositing the objects. The entire learning process is unsupervised and end-to-end. In experiments, in addition to generation quality, we also demonstrate that the learned representation permits object-wise manipulation and novel scene generation, and generalizes to various settings. Results can be found on our project website: https://sites.google.com/view/roots3d

==> code.tex <==
\begin{algorithm}[t]
% \footnotesize
\caption{ROOTS Encoder}
\label{algo:enc}
\begin{algorithmic}
    \ENSURE  $f_{xy}^c=$ MLP, \hspace{1mm} $f_{\text{order-invariant}}^c=\sum f_{xy}^c$ 
    \REQUIRE $h_0^x$, $\{ \th_0^{k} \}_{k\in [K]}$, $\tX_0$, $\{ \tv_0^{k} \}_{k\in [K]}$
    % \STATE \# \textit{Scene Encoder}
    \STATE Context encoding: $\rvr = f_\text{ctx\_enc}(\gC)$
    \STATE Get object position and presence in 3D world coordinate: $\rvz_{ijk}^\where, \rvz_{ijk}^\pres = \rvr$
    % \STATE \# \textit{Object Grouping}
    \FOR {$n=(i,j,k)$ such that $\rvz_{ijk}^\pres = 1$ \textbf{parallel}} 
        \FOR {each context $c \in \gC$ \textbf{parallel}} 
            \STATE Obtain attended image region $\rvx_{n,c}^\att \subset \rvx_c$ using Attention-by-Perspective-Projection
        \ENDFOR
        \STATE Obtain object context $\gC_n = \{\rvx_{n,c}^\att, \rvv_{c}\}$ 
        % by collecting attended image regions matching to object $n$
        \STATE Obtain 3D appearance representation for object $n$: $\rvz_{n}^\what = \text{GQN}_\text{enc}(\gC_n)$.
        \STATE \textbf{return} $\rvz_n^\pres, \rvz_n^\where, \rvz_n^\what$
    \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
% \footnotesize
\caption{ROOTS Encoder}
\label{algo:enc}
\begin{algorithmic}
    \ENSURE
    \REQUIRE
    % \STATE \# \textit{Scene Encoder}
    \STATE Obtain Geometric Volume Feature Map $\bm{r} = f_\mathrm{ctx\_enc}(\gC) \in \R^{N_x \times N_y \times N_z \times d}$
    \FOR {\textbf{each} $(i,j,k) \in [N_x] \times [N_y] \times [N_z]$ \textbf{parallel}}
        \STATE Infer object presence and position in 3D world coordinates: $\rz_{ijk}^\pres, \rvz_{ijk}^\where \sim f_{\pres, \where}(\bm{r})$
    \ENDFOR
    \STATE Obtain the number of objects $N = {\textstyle\sum}_{ijk}\,\rz_{ijk}^\pres$
    \STATE 
    % \STATE \# \textit{Object Grouping}
    \FOR {\textbf{each} $n \in [N]$ \textbf{parallel}}
        \FOR {\textbf{each} context $(\rvx_c, \rvv_c) \in \gC$ \textbf{parallel}}
            \STATE Obtain attended image region $\rvx_{n,c}^\att \subset \rvx_c$ using Attention-by-Perspective-Projection
        \ENDFOR
        \STATE Obtain object-level context $\gC_n = \{\rvx_{n,c}^\att, \rvv_{c}\}$ 
        % by collecting attended image regions matching to object $n$
        \STATE Infer 3D appearance representation for object $n$: $\rvz_n^\what \sim \GQN_\enc({\gC}_n)$.
        \STATE \textbf{return} $\rvz_n^\pres, \rvz_n^\where, \rvz_n^\what$
    \ENDFOR
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[t]
\footnotesize
\caption{ROOTS Decoder}
\label{algo:dec}
\begin{algorithmic}
    \ENSURE
    \REQUIRE
    \FOR {\textbf{each} $n \in [N]$ \textbf{parallel}}
        \STATE Object-level context encoding: $\bm{r}_n^\att = f_\mathrm{obj\_ctx\_enc}(\gC_n)$
        \FOR {\textbf{each} query viewpoint $\rvv_q$}
            \STATE Decode 3D appearance $\rvz_{n}^\what$ into 2D image patch $\rvo_{n,q}^\what = \GQN_\dec(\texttt{concat}[\rvz_n^\what, \bm{r}_n^\att], \rvv_q)$
            \STATE Obtain object-specific image layer $\hat{\rvx}_{n,q}$ and transparency map $\bm{\alpha}_{n,q}$ using Attention-by-Perspective-Projection
        \ENDFOR
    \ENDFOR
    \STATE Composite the final image $\hat{\rvx}_{q} = {\textstyle\sum}_{n=1}^{N}\,\bm{\alpha}_{n,q} \odot \hat{\rvx}_{n,q}$
\end{algorithmic}
\end{algorithm}
